Advancing Geometry with AI: Multi-agent Generation of Polytopes

Polytopes are one of the most primitive concepts underlying geometry. Discovery and study of polytopes with complex structures provides a means of advancing scientific knowledge. Construction of polytopes with specific extremal structure is very difficult and time-consuming. Having an automated tool for the generation of such extremal examples is therefore of great value. We present an Artificial Intelligence system capable of generating novel polytopes with very high complexity, whose abilities we demonstrate in three different and challenging scenarios: the Hirsch Conjecture, the k-neighbourly problem and the longest monotone paths problem. For each of these three problems the system was able to generate novel examples, which match or surpass the best previously known bounds. Our main focus was the Hirsch Conjecture, which had remained an open problem for over 50 years. The highly parallel A.I. system presented in this paper was able to generate millions of examples, with many of them surpassing best known previous results and possessing properties not present in the earlier human-constructed examples. For comparison, it took leading human experts over 50 years to handcraft the first example of a polytope exceeding the bound conjectured by Hirsch, and in the decade since humans were able to construct only a scarce few families of such counterexample polytopes. With the adoption of computer-aided methods, the creation of new examples of mathematical objects stops being a domain reserved only for human expertise. Advances in A.I. provide mathematicians with yet another powerful tool in advancing mathematical knowledge. The results presented demonstrate that A.I. is capable of addressing problems in geometry recognized as extremely hard, and also to produce extremal examples different in nature from the ones constructed by humans.

==> old_stuff_inactive.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     OLD    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Old introduction}
The advancement of science is based on observations. A biologist observes specimens of living organisms and advances their field by studying them. Physics is advanced by observing phenomena occurring in the world. Mathematics is advanced by observing and studying abstract objects. Looking at the development of Physics we can see how with its progress the naturally observed phenomena stopped being sufficient and the need arose for creation of artificial experimental devices, such as the famous hadron colliders. The same holds true for mathematics. 
Geometry is one of the most ancient and most fundamental domains of mathematics. An essential component of the scientific progress is discovery of the new objects. Polytopes are one of the most foundational objects in geometry and have been studied for thousands of years. Still, we are far from understanding their geometry, as despite their basic nature their properties can be extremely advanced.
 Discovery and study of polytopes with complex structures provides means of advancing scientific knowledge. Such "extremal examples" are very difficult to find, hence having an automated tool for their generation can be of great value. In this paper we present a transformer-based Artificial Intelligence system capable of generating novel polytopes with very high complexity.
 This system can be targeted towards different scenarios by choosing a different fitness metric, while using the same core codebase. 
 For this paper we chose three different challenging scenarios: the Hirsch Conjecture, the $k$-neighbourly problem and the longest monotone paths problem. For each of these three problems the system was able to generate novel examples, that  surpass the best previously known results.\\
Our main focus was the Hirsch Conjecture. In this case the AI showed its advantages both in terms of quality and quantity. The AI system presented in this paper was able to generate millions of examples in less than a month time, with many of them exceeding SOTA and possessing properties never observed before. For comparison, it took top human experts over 50 years to construct the first example, and in 10 years humans were able to construct less than 10 such polytopes.
\adam{The intro is good but I feel it could be better. We need to do a better job marketing.}

\begin{abstract}
    Polytopes -- like triangles, squares, cubes and dodecahedrons -- are fundamental objects in mathematics and computer science. The generation of interesting ``extremal'' examples in high-dimension is a major unsolved problem. Known examples can take human experts decades for their discovery, and in several important cases only a few interesting examples are known. We present an Artificial Intelligence system capable of generating novel polytopes with very high complexity, whose abilities we demonstrate in three different challenging scenarios in polytope theory: the celebrated Hirsch Conjecture, the $k$-neighbourly problem and the longest monotone paths problem. In each of these three problems our system was able to generate novel examples, which match or surpass the best previously known constructions. Moreover, the AI generated examples display characteristics not present in known human constructions.
\end{abstract}


\section{The Hopper algorithm}
\subsection{Overview}
The goal of the Hopper algorithm is to create examples of polytopes with a user-specified desired property $\varrho$. In order for a Hopper to work a verification function $\nu$ needs to be provided which for any polytope $P$ yields a value TRUE if $P$ has the property $\varrho$ and FALSE if it does not. Additionally, a fitness function $f$ is needed. This function can be thought of as a continuous approximation of the binary function $\nu$. If for two polytopes $P_1$ and $P_2$ there holds $f(P_1) < f(P_2)$ then the polytope $P_2$ is "closer to having property $\varrho$ than $P_1$".\\
The Hopper uses the concept of a population refinement. On initialization a collection of polytopes is created using a suitable random procedure. Upon those a collection of agents works using a work-stealing strategy. Each agent picks up a polytope and attempts to modify it using an action chosen  from the list of available actions, by using a transformer-based neural network.\\
The Hopper is not a Reinforcement Learning algorithm in the conventional sense, nevertheless we are going to use the state space/action space terminology.

 
%%%%%%%%%%   STATE SPACE   %%%%%%%%%%
\subsection{State space}
The "raw" natural state space for the Hopper to operate in is a space of all polytopes with $k$ vertices in $d$-dimensional Euclidean space $\RR^d$. Such space is an $n \cdot d$ dimensional manifold. It is usually more advantageous to work with discrete state spaces. Thus it is desirable to reduce the state space into a discrete set of equivalence classes whose members are indistinguishable from the perspective of the property $\varrho$. In all three problems considered in this paper the natural equivalence between the polytopes is in terms of their connection graphs.


%%%%%%%%%%   ACTION SPACE   %%%%%%%%%%
\subsection{Action space and the transformer-based brain}
\label{subs::action_space}
A natural primitive action when working with polytopes is a modification of one of the vertices by shifting it by a vector. Such choice makes the action space continuous, with clusters (being polytopes themselves) of actions yielding an equivalent outcome. Hence in this paper we use a discretization. We leverage the existence of a natural partition of the ($d$-dimensional) Euclidean space $\RR^d$ containing the polytope $P$ by all hyperplanes determined by $d-1$ subsets of the set $V = \{v_i \}$  of vertices of $P$. Those hyperplanes partion the space $\RR^d$ into a collection of mutually disjoint polytopes $\{V_{\iota}\}$. Thus our action space will be defined as a set of pairs $(i, \iota)$. Choosing an action $(i, \iota)$ means: we take a vertex $v_i$ of polytope $P$ and we replace it with some point inside the partition cell $\iota$. Such action we named a {\it hop}, hence the name of the main algorithm.\\
Two issues here require clarification. The first is - many of such actions can lead to a geometric degeneracy of the polytope . A vertex could simply be moved into the interior of $P$ in such manner. In other case some other vertices might end up not being vertices but interior points. Also - some huge disproportions in shape may result, leading to numerical difficulties. The second issue is related to the choice of the interior point inside the partition cell $\iota$. It is easy to show that from the perspective of the connection graph each such choice is equivalent. Nevertheless, the choices can have an impact on the efficiency of the numerical representation. Both of those issues are addressed by a number of techniques which are briefly discussed in \ref{supp::stability} and \ref{supp::geometry}.
Initially the actions are chosen uniformly at random. As the work progresses, more and more knowlegde can be gained. The agent are equipped with a "brain" $\beta$ that allows it to happen. The architecture of that brain - a transformer-based neural network - is described in detail in~\ref{supp::hopper_brain_architecture}. The brain takes as an input a pair $(P, h)$ a polytope and a hyperplane and outputs a floating point number representing a likelihood of hyperplane $h$ being a part of a boundary of a successful hop region (see Algorithm~\ref{alg::individual_agent}). Speaking in the language of Reinforcement Learning, the brain $\beta$ corresponds to the policy, which we are improving over time by learning from our experiences.

%%%%%%%%%%   ACTIONS of an AGENT   %%%%%%%%%%
\subsection{Actions of an agent}
An individual agent operates in a work stealing mode repeating the following sequence of operations in an infinite loop until a global stop signal is issued.
\begin{itemize}[align=left, leftmargin=*] 
    \item [(Read/Init)] Take a polytope - randomly generated or by means of reading
    \item [(Process)] Try to improve the polytope using available actions
    \item [(Write/Discard)] If improvement achieved write to the shared repository
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%     AGENT ALGORITHM    %%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]\caption{Hopper algorithm - individual agent}
\label{alg::individual_agent}
\begin{center}
\begin{algorithmic}[1]
% \item[\textbf{Parameters:}]
\Require Polytope $P \in \RR^d$, represented as a $n \times d$ matrix $V$ of vertices. Fitness function $f$. Likelihood function $\beta$ \footnotemark.
\Ensure The given vertices span $P$ properly - no vertex is inside a convex hull of other vertices
% \State \textbf{assert } Eq. (\ref{eq:tensor_rank_decomposition}) holds, where $u_r, v_r, w_r$ are vectorized forms of $U_r, V_r, W_r$
%\Header{Compute hyperplanes}
\GMSalgoHeader{Compute hyperplanes}
\State $\mathcal{H} = \emptyset$ % \Comment{Compute hyperplanes}
\For{ all $\{ v_{1}, \ldots v_{d}\} \subseteq V$ sets of distinct $d$ vertices}
\State $\mathcal{H}.{\rm append}(h)$, $h$ - equation of a hyperplane containing $\{ v_{1}, \ldots v_{d-1}\}$
\State Compute probability distribution $\pi$ on hyperplanes in $\mathcal{H}$ by computing likelihoods of each $h$ using likelihood function $\beta$ (see~\ref{subs::action_space}) and normalizing them by dividing by their sum. 
\EndFor
% \EndHeader%
\GMSalgoHeader{Construct hop target $c$}
% \Header{Construct hop target $c$}
\State $\mathcal{A} = \emptyset$ % \Comment{Construct action}
\State Sample $d+1$ equations $h_1, \ldots h_{d+1}$ from $\mathcal{H}$ according to $\pi$ and change them to inequalities $\chi_1, \ldots, \chi_{d+1}$, choosing directions of the inequalities  such that the feasible set is nonempty.
If the feasible set is not bounded or the shape violates geometric constrains, discard $\chi_1, \ldots, \chi_{d+1}$ and sample again.
\State $\mathcal{A} \leftarrow \chi_1, \ldots, \chi_{d+1}$
\State Find $(c, r)$ - the center and radius of the largest ball inscribed in the polytope defined by $\mathcal{A}$.
\While{exists $h \in \mathcal{H}$ such that ${\rm dist}(h, c) < 0.8 * r$}
\State $\mathcal{A}.{\rm append}(h)$
\State Recompute $(c, r)$
\EndWhile
% \EndHeader
\GMSalgoHeader{Construct list of candidates}
% \Header{Construct list of candidates}
\State C = []
\For{$v \in V$}
\State Construct polytope $P'$ by replacing $v$ with $c$
\If{$P'$ satisfies admissibility criteria}
\State $C.{\rm append}(P')$
\EndIf
\EndFor
% \EndHeader
\GMSalgoHeader{Evaluate candidates}
% \Header{Evaluate candidates}
\For{$\varrho \in C$}
\If{$f(\varrho) < f(P)$}
\State $C.{\rm delete}(\varrho)$
\EndIf
\EndFor
% \EndHeader
\State \Return $\argmax\limits_f C$
\end{algorithmic}
\end{center}
\end{algorithm}
\footnotetext{{Likelihood function $\beta$ is an output of a neural network being trained in an online fashion. For more details see Appendix~\ref{supp::hopper_brain_architecture}.}}

%%%%%%%%%%%%%%%%%%%    END AGENT ALGORITHM    %%%%%%%%%%%%%%%%%%%


% \subsection{Hopper brain}
% \greg{Needs to go somewhere where it makes sense. Circular dependency currently, I use algorithm format to avoid verbose talk about hyperplanes, but I need hyperplanes to talk about the brain. Idea: mention brain in the action space section saying "we use neural network to give distribution over actions" and defer details to algorithm.}\adam{Yes I think this would be a good way of doing it. I would not do it in the action space (that just defines the magic table), but rather in the next section where you talk about how the agent performs the actions. In point iii) there I would emphasize that by "random", we really mean random according to a distribution given by a neural network. I would also add a sentence here saying that this network is the brain of the Hopper that needs to be trained, and that you will explain it in more detail later. We should also make a big deal about how this brain was key to making Hopper work.}



%%%%%%%%%%   KNOWLEDGE DISTILLATION   %%%%%%%%%%
\subsection{Knowledge distillation}
\label{subs::knowledge_distillation}
The Hopper consists of a collection of agents. The agents work independently, but they share the data repository. Each agent accesses the repository. In case the repository is empty, the agent generates a random polytope and starts working on it. Otherwise the agent makes a decision: with a probability $p_{{\rm read}}$ it copies (not deleting) a polytope from the repository or with a probability $(1-p_{{\rm read}})$ generates a random polytope. If the agent manages to obtain an improvement of the polytope it is working on, the improved polytope is inserted into the repository. Each inserted polytope has an "importance score" attached, which is a combination of the fitness function value and factors like the history of improvements, number of failures to improve the polytope etc.\\
If the size of the repository exceeds the maximum allowed size, the polytopes are discarded according to their importance score in a slightly randomized manner (for some technical details see Supplementary Material~\ref{supp::shared_repository}).


\subsection{Collection of agents}


% \subsection{Hypeparameters}
% \greg{Do we need this section?}\adam{Maybe a very very short one -- the paper is already going to be too long, and the other sections are more important}\greg{I am inclined to ditch it at some point, keeping it for the time being.}
% \begin{itemize}
%     \item [$p_{{\rm read}}$] With probability $p_{{\rm read}}$ read from repository, with probability $1-p_{read}$ random init
%     \item [] Stopping time / stopping \# of iterations
%     \item [] Repository size limit
% \end{itemize}

Polytopes may be described in two different ways. In the first, one specifies a list of vertices and takes their convex hull (the vertex description). In the second, one specifies a list of inequalities describing the faces and takes their intersection (the face description). For example, the cube may be described either as the convex hull of its 8 vertices $(\pm 1, \pm 1, \pm 1)$ or as the region where all coordinates lie between -1 and 1. One major source of difficulty is that these two descriptions can have drastically different complexity: the $n$-dimensional cube has $2n$ faces, but $2^n$ vertices, hence its face description is exponentially more efficient than its vertex description. 

A polytope has faces of all dimensions between 0 and $n-1$ (vertices are dimension 0, edges dimension 1 etc.) and their incidence relations determines the lattice of faces (see Figure 1). We care exclusively about the combinatorial type of polytopes, in other words we only care about the lattice of faces. Two important graphs arise from a polytope: the vertex/edge graph has nodes and edges corresponding to the vertices and edges of the polytope; the facet/ridge graph has nodes and edges corresponding to the facets (codimension 1 faces) and ridges (codimension 2 faces).

\geordie{Not exactly sure how much detail we need here. Will return to this once the algorithm section is in better shape.}
